Rethinking the Bounds of LLM Reasoning: Are Multi-Agent Discussions the Key?

Recent progress in LLMs discussion suggests that multi-agent discussion improves the reasoning abilities of LLMs. In this work, we reevaluate this claim through systematic experiments, where we propose a novel group discussion framework to enrich the set of discussion mechanisms. Interestingly, our results show that a single-agent LLM with strong prompts can achieve almost the same performance as the best existing discussion approach on a wide range of reasoning tasks and backbone LLMs. We observe that the multi-agent discussion performs better than a single agent only when there is no demonstration in the prompt. Further study reveals the common interaction mechanisms of LLMs during the discussion.

==> latex/6-relatedwork.tex <==
\section{Related Work}
\subsection{Large language models $\llm$}
With the advent of large language models (LLMs) like GPT-3 \citep{gpt3}, chatGPT \citep{chatgpt}, GPT-4 \citep{gpt4}, Llama series \citep{llama, llama2} and PaLM 2 \citep{palm2}, prompt engineering is a burgeoning field that focuses on optimizing the output of language models by crafting effective input prompts.

\syc{Bard, Germini}.

\subsection{Prompt decorator $p(\cdot; \task, \llm)$ for reasoning}
Numerous advancements have been made in the field of improving reasoning abilities of LLMs with prompt engineering. Chain of Thought (CoT) \citep{cot, cot0} is a linear problem-solving approach where each step builds upon the previous one. \citet{firstms} propose to apply CoT to multi-step reasoning tasks. To automate the CoT, Auto-CoT \citep{autop} constructs demonstrations by sampling diverse questions and generating reasoning chains. Active-Prompt \citep{activep} aims to select the most uncertain questions for task-specific annotations. Other prompt strategies include PS prompt \citep{pas} which divides task into subtasks then solve them, effective GoT \citep{eGoT} which models human thought processes as a graph rather than a chain, Natural Program \citep{np} which helps to improve the deductive reasoning tasks, re-reading prompt \citep{reread} which revisits the question information embedded within input prompts.

\subsection{Mechanism $\mech$ for reasoning}\label{sec:related-mechanism}
In addition to focusing on the design of prompts themselves, some works incorporate different mechanisms to assist language models in reasoning. 

The design directions of these mechanisms include: 
1. Breaking down the reasoning process into multiple stages, with possible verification at each stage. 
2. Optimizing the reasoning process via ensemble methods.
3. Iteratively prompting the model for reflection and correction. 
4. Utilizing external tools to aid in reasoning. These approaches aim to enhance the overall reasoning capabilities of language models by introducing additional support and guidance throughout the process.\par
\noindent\textbf{Break Down the Reasoning Process into Multiple Stages.}
Self-Polish \citep{sp} make models to progressively refine given problems with multiple stages of prompts. Additionally, some works \citep{decomp, mes, succ, cr} study over decomposing the tasks into smaller tasks, and use an individual prompt to solve each subtask.\par
\noindent\textbf{Optimize the Reasoning Process via Ensemble Methods.}
Tree of Thoughts (ToT) \citep{tot} expands on the reasoning process by considering multiple paths of reasoning and self-evaluating choices. Graph of Thoughts (GoT) \citep{got} further advances this by modeling information as an arbitrary graph, enabling complex networks of thoughts. And some works propose to first sample reasoning pathsvthen vote for the best one, including self-consistency \citep{cot-sc} and step-aware verifier \citep{step-verifier}. Discussion Engineering is also one category of ensemble methods. We will leave it to section \ref{sec:de} for further introduction.\par
\noindent\textbf{Iteratively Prompt the Model for Reflection and Correction.} These works \citep{star, sv, reflexion, sr, sd, rcot} are mainly based on iteratively asking model to find the mistakes or inconsistencies among previous reasoning steps or the knowledge, then solve them one by one. \par
\noindent\textbf{Utilize External Tools or Knowledge to Aid in Reasoning.} Mind's Eye \citep{mindeye} proposes to use physical simulator to help models reason in the physical world. There are also other works \cite{chameleon, mathprompter} will equip models with tools to solve problems. Further more, some works like MemPrompt \citep{memprompt} and LogicSolver \cite{logicsolver} use external knowledge to assist LLMs with reasoning.\par

\subsection{Discussion Engineering - A Subset of Mechanism $\mech$} \label{sec:de}
Self-organized discussion involves multi-agent interactions, where agents spontaneously navigate the entire discussion process and reach a conclusion based on their assigned roles, discussion topics, and framework. Discussion Engineering, a subset of mechanism design $\mech$, focuses on defining crucial components of the discussion framework in self-organized discussions. This includes the discussion process algorithm, roles, utilized Language Models (LLMs), and prompt decorators $p(\cdot; \task, \llm)$ employed at different discussion stages. By leveraging the input interface of an LLM, Discussion Engineering simulates the information exchange between agents and generates corresponding outputs to mimic their speech during ongoing discussions, enabling downstream task-oriented mechanisms.

\noindent\textbf{Recent Works.} Recent progress has been made in the design of Discussion Engineering. The Multi-Agent Debate framework, introduced by \cite{debate}, establishes a mechanism for symmetric discussions among participants (agents). In this framework, agents begin in a consistent state but diverge in their initial answers through spontaneous adversarial generation of Language Models (LLMs). Subsequently, the agents engage in debate to reach a consensus. During the same period, the MAD (Multi-Agent Debate) framework \citep{mad} introduces an asymmetric mechanism design. It assigns different roles (debater and judge) asymmetrically and utilizes different prompt decorators for similar roles (affirmative and negative sides). Other similar works include \cite{chan2023chateval}. Also, the ReConcile framework \citep{reconcile} exemplifies an asymmetric discussion mechanism by involving different LLMs and using distinct prompt decorators with varying convincing samples for each agent. To understand discussion more deeply, \cite{expd} try to explain such collaboration mechanism in a social psychology view. 

\noindent\textbf{Exploration Gaps: Discussion Frameworks, Prompt Decorators, and Mechanism Design.} Most of the existing works in this field primarily focus on evaluating the effectiveness of their own designed discussion frameworks or merely discussing the impact of different settings on the performance of these frameworks. However, there is a limited exploration of the potential effects that rich prompt decorator designs may have on the discussion process. Furthermore, there is currently a lack of unified definitions and discussions on Discussion Engineering and mechanism design based on language models. Additionally, little research has been conducted on examining the symmetry of mechanisms within discussions. Overall, more research is needed to understand the potential effects of rich prompt decorators and definition of mechanism design and symmetry.

==> latex/acknowledge.tex <==
\section*{Acknowledgements}

Zihao Wang thanks Mr. Datong Zhou from The Pennsylvania State University for the discussion on symmetry.
